Particle-Gibbs Sampling For Bayesian Feature Allocation Models

Bayesian feature allocation models are a popular tool for modelling data with a combinatorial latent structure. Exact inference in these models is generally intractable and so practitioners typically apply Markov Chain Monte Carlo (MCMC) methods for posterior inference. The most widely used MCMC strategies rely on an element wise Gibbs update of the feature allocation matrix. These element wise updates can be inefficient as features are typically strongly correlated. To overcome this problem we have developed a Gibbs sampler that can update an entire row of the feature allocation matrix in a single move. However, this sampler is impractical for models with a large number of features as the computational complexity scales exponentially in the number of features. We develop a Particle Gibbs sampler that targets the same distribution as the row wise Gibbs updates, but has computational complexity that only grows linearly in the number of features. We compare the performance of our proposed methods to the standard Gibbs sampler using synthetic data from a range of feature allocation models. Our results suggest that row wise updates using the PG methodology can significantly improve the performance of samplers for feature allocation models.

==> tables/latex/friedman_test/dpf_annealing_power.tex <==
\toprule
Metric & Relative log density &             RMSE \\
Time   &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{DPF}{annealing powers}} \label{tab:friedman_dpf_annealing_power} \\ 
\endlastfoot
10.0   &      \textbf{0.0000} &           0.0028 \\
100.0  &      \textbf{0.0000} &  \textbf{0.0000} \\
1000.0 &      \textbf{0.0000} &  \textbf{0.0000} \\


==> tables/latex/friedman_test/dpf_num_particles.tex <==
\toprule
Metric & Relative log density &             RMSE \\
Time   &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{DPF}{number of particles}} \label{tab:friedman_dpf_num_particles} \\ 
\endlastfoot
10.0   &      \textbf{0.0000} &  \textbf{0.0000} \\
100.0  &      \textbf{0.0000} &  \textbf{0.0000} \\
1000.0 &      \textbf{0.0000} &  \textbf{0.0000} \\


==> tables/latex/friedman_test/dpf_test_path.tex <==
\toprule
Metric & Relative log density &             RMSE \\
Time   &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{DPF}{test paths}} \label{tab:friedman_dpf_test_path} \\ 
\endlastfoot
10.0   &      \textbf{0.0000} &  \textbf{0.0000} \\
100.0  &      \textbf{0.0000} &  \textbf{0.0000} \\
1000.0 &      \textbf{0.0000} &  \textbf{0.0000} \\


==> tables/latex/friedman_test/lfrm_finite_20.tex <==
\toprule
Metric & Relative log density & Reconstruction error \\
Time    &                      &                      \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLFRMCaption{K=20}} \label{tab:friedman_lfrm_finite_20} \\ 
\endlastfoot
100.0   &      \textbf{0.0004} &               0.0031 \\
1000.0  &               0.0031 &               0.4296 \\
10000.0 &               0.7886 &               0.8229 \\


==> tables/latex/friedman_test/lfrm_finite_5.tex <==
\toprule
Metric & Relative log density & Reconstruction error \\
Time    &                      &                      \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLFRMCaption{K=5}} \label{tab:friedman_lfrm_finite_5} \\ 
\endlastfoot
100.0   &      \textbf{0.0000} &               0.0030 \\
1000.0  &      \textbf{0.0000} &               0.0264 \\
10000.0 &      \textbf{0.0000} &               0.0151 \\


==> tables/latex/friedman_test/lfrm_ibp_20.tex <==
\toprule
Metric & Relative log density & Reconstruction error \\
Time     &                      &                      \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLFRMCaption{K=20 and an IBP prior}} \label{tab:friedman_lfrm_ibp_20} \\ 
\endlastfoot
100.0    &               0.0094 &      \textbf{0.0004} \\
1000.0   &               0.0571 &               0.4949 \\
100000.0 &               0.4328 &               0.6771 \\


==> tables/latex/friedman_test/lg_finite_20.tex <==
\toprule
Metric & Relative log density &             RMSE \\
Time    &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLGCaption{K=20}} \label{tab:friedman_lg_finite_20} \\ 
\endlastfoot
100.0   &      \textbf{0.0000} &  \textbf{0.0000} \\
1000.0  &      \textbf{0.0000} &  \textbf{0.0000} \\
10000.0 &      \textbf{0.0000} &  \textbf{0.0000} \\


==> tables/latex/friedman_test/lg_finite_5.tex <==
\toprule
Metric & Relative log density &             RMSE \\
Time    &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLGCaption{K=5}} \label{tab:friedman_lg_finite_5} \\ 
\endlastfoot
100.0   &      \textbf{0.0000} &  \textbf{0.0000} \\
1000.0  &      \textbf{0.0000} &  \textbf{0.0000} \\
10000.0 &      \textbf{0.0000} &  \textbf{0.0000} \\


==> tables/latex/friedman_test/lg_ibp_20.tex <==
\toprule
Metric & Relative log density &             RMSE \\
Time     &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLGCaption{K=20 and an IBP prior}} \label{tab:friedman_lg_ibp_20} \\ 
\endlastfoot
100.0    &      \textbf{0.0000} &  \textbf{0.0000} \\
1000.0   &      \textbf{0.0000} &  \textbf{0.0000} \\
100000.0 &      \textbf{0.0000} &  \textbf{0.0000} \\


==> tables/latex/friedman_test/pg_annealing_power.tex <==
\toprule
Metric & Relative log density &             RMSE \\
Time   &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{PG}{annealing powers}} \label{tab:friedman_pg_annealing_power} \\ 
\endlastfoot
10.0   &      \textbf{0.0000} &  \textbf{0.0000} \\
100.0  &      \textbf{0.0000} &  \textbf{0.0000} \\
1000.0 &      \textbf{0.0000} &  \textbf{0.0000} \\


==> tables/latex/friedman_test/pg_num_particles.tex <==
\toprule
Metric & Relative log density &             RMSE \\
Time   &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{PG}{number of particles}} \label{tab:friedman_pg_num_particles} \\ 
\endlastfoot
10.0   &      \textbf{0.0000} &  \textbf{0.0000} \\
100.0  &      \textbf{0.0000} &           0.0060 \\
1000.0 &      \textbf{0.0000} &           0.0393 \\


==> tables/latex/friedman_test/pg_resample_threshold.tex <==
\toprule
Metric & Relative log density &             RMSE \\
Time   &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{PG}{resampling thresholds}} \label{tab:friedman_pg_resample_threshold} \\ 
\endlastfoot
10.0   &      \textbf{0.0000} &  \textbf{0.0000} \\
100.0  &      \textbf{0.0000} &           0.0581 \\
1000.0 &      \textbf{0.0000} &  \textbf{0.0001} \\


==> tables/latex/friedman_test/pg_test_path.tex <==
\toprule
Metric & Relative log density &             RMSE \\
Time   &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{PG}{test paths}} \label{tab:friedman_pg_test_path} \\ 
\endlastfoot
10.0   &      \textbf{0.0000} &  \textbf{0.0000} \\
100.0  &      \textbf{0.0000} &  \textbf{0.0000} \\
1000.0 &      \textbf{0.0000} &  \textbf{0.0000} \\


==> tables/latex/friedman_test/pyclone_finite_12.tex <==
\toprule
Metric & Relative log density & B-Cubed F-Measure \\
Time    &                      &                   \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanPyCloneCaption{D=10 and K=12}} \label{tab:friedman_pyclone_finite_12} \\ 
\endlastfoot
100.0   &      \textbf{0.0000} &   \textbf{0.0000} \\
1000.0  &      \textbf{0.0000} &   \textbf{0.0000} \\
10000.0 &      \textbf{0.0000} &   \textbf{0.0000} \\


==> tables/latex/friedman_test/pyclone_finite_4.tex <==
\toprule
Metric & Relative log density & B-Cubed F-Measure \\
Time    &                      &                   \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanPyCloneCaption{D=4 and K=4}} \label{tab:friedman_pyclone_finite_4} \\ 
\endlastfoot
100.0   &      \textbf{0.0000} &   \textbf{0.0000} \\
1000.0  &      \textbf{0.0000} &   \textbf{0.0000} \\
10000.0 &      \textbf{0.0000} &   \textbf{0.0000} \\


==> tables/latex/friedman_test/pyclone_finite_8.tex <==
\toprule
Metric & Relative log density & B-Cubed F-Measure \\
Time    &                      &                   \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanPyCloneCaption{D=10 and K=8}} \label{tab:friedman_pyclone_finite_8} \\ 
\endlastfoot
100.0   &      \textbf{0.0000} &   \textbf{0.0000} \\
1000.0  &      \textbf{0.0000} &   \textbf{0.0000} \\
10000.0 &      \textbf{0.0000} &   \textbf{0.0000} \\


==> tables/latex/nemenyi_test/dpf_annealing_power.tex <==
\toprule
     &     &     & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{RMSE} \\
     &     &     &      Mean difference &          P-Value & Mean difference & P-Value \\
Time & Param 1 & Param 2 &                      &                  &                 &         \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{DPF}{annealing powers}} \label{tab:nemenyi_dpf_annealing_power} \\ 
\endlastfoot
\multirow{6}{*}{10} & \multirow{3}{*}{0.0} & 1.0 &              -0.1168 &           0.0227 &          0.0676 &      NS \\
     &     & 2.0 &              -0.1317 &           0.1023 &          0.0702 &      NS \\
     &     & 3.0 &     \textbf{-0.1392} &  \textbf{0.0002} &          0.0842 &      NS \\
\cline{2-7}
     & \multirow{2}{*}{1.0} & 2.0 &              -0.0149 &           0.9820 &          0.0026 &      NS \\
     &     & 3.0 &              -0.0224 &           0.7219 &          0.0166 &      NS \\
\cline{2-7}
     & 2.0 & 3.0 &              -0.0075 &           0.3735 &          0.0140 &      NS \\
\cline{1-7}
\multirow{6}{*}{100} & \multirow{3}{*}{0.0} & 1.0 &              -0.0108 &           0.9996 &          0.0429 &  0.9667 \\
     &     & 2.0 &              -0.0034 &           0.9946 &          0.0387 &  0.7514 \\
     &     & 3.0 &              -0.0149 &           0.9874 &          0.0622 &  0.4032 \\
\cline{2-7}
     & \multirow{2}{*}{1.0} & 2.0 &               0.0074 &           0.9751 &         -0.0043 &  0.9820 \\
     &     & 3.0 &              -0.0041 &           0.9982 &          0.0193 &  0.8066 \\
\cline{2-7}
     & 2.0 & 3.0 &              -0.0114 &           0.8970 &          0.0236 &  0.9820 \\
\cline{1-7}
\multirow{6}{*}{1000} & \multirow{3}{*}{0.0} & 1.0 &              -0.0076 &           0.9999 &          0.0200 &  0.9999 \\
     &     & 2.0 &              -0.0168 &           0.6912 &         -0.0073 &  0.8319 \\
     &     & 3.0 &              -0.0191 &           0.9446 &          0.0342 &  0.9915 \\
\cline{2-7}
     & \multirow{2}{*}{1.0} & 2.0 &              -0.0093 &           0.7797 &         -0.0272 &  0.7514 \\
     &     & 3.0 &              -0.0116 &           0.9751 &          0.0142 &  0.9982 \\
\cline{2-7}
     & 2.0 & 3.0 &              -0.0023 &           0.9820 &          0.0415 &  0.5624 \\






==> tables/latex/nemenyi_test/dpf_num_particles.tex <==
\toprule
     &   &    & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{RMSE} \\
     &   &    &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Param 1 & Param 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{DPF}{number of particles}} \label{tab:nemenyi_dpf_num_particles} \\ 
\endlastfoot
\multirow{15}{*}{10} & \multirow{5}{*}{10} & 100 &      \textbf{2.4108} &  \textbf{0.0000} &  \textbf{-0.4485} &  \textbf{0.0000} \\
     &   & 2 &               0.0585 &           0.4064 &           -0.0628 &           0.5028 \\
     &   & 20 &               0.0847 &           1.0000 &            0.0521 &           0.9051 \\
     &   & 5 &              -0.0195 &           1.0000 &            0.0348 &           0.9290 \\
     &   & 50 &      \textbf{1.1853} &  \textbf{0.0000} &           -0.1525 &           0.0017 \\
\cline{2-7}
     & \multirow{4}{*}{100} & 2 &     \textbf{-2.3523} &  \textbf{0.0000} &   \textbf{0.3856} &  \textbf{0.0000} \\
     &   & 20 &     \textbf{-2.3261} &  \textbf{0.0000} &   \textbf{0.5006} &  \textbf{0.0000} \\
     &   & 5 &     \textbf{-2.4303} &  \textbf{0.0000} &   \textbf{0.4833} &  \textbf{0.0000} \\
     &   & 50 &              -1.2254 &           0.0477 &   \textbf{0.2960} &  \textbf{0.0001} \\
\cline{2-7}
     & \multirow{3}{*}{2} & 20 &               0.0262 &           0.5776 &            0.1149 &           0.0385 \\
     &   & 5 &              -0.0780 &           0.2976 &            0.0977 &           0.0477 \\
     &   & 50 &      \textbf{1.1269} &  \textbf{0.0000} &           -0.0897 &           0.3834 \\
\cline{2-7}
     & \multirow{2}{*}{20} & 5 &              -0.1042 &           0.9995 &           -0.0173 &           1.0000 \\
     &   & 50 &      \textbf{1.1007} &  \textbf{0.0000} &  \textbf{-0.2046} &  \textbf{0.0000} \\
\cline{2-7}
     & 5 & 50 &      \textbf{1.2048} &  \textbf{0.0000} &  \textbf{-0.1873} &  \textbf{0.0000} \\
\cline{1-7}
\multirow{15}{*}{100} & \multirow{5}{*}{10} & 100 &               0.0153 &           0.7872 &            0.0301 &           0.9703 \\
     &   & 2 &               0.0090 &           0.9947 &           -0.1183 &           0.1919 \\
     &   & 20 &              -0.0077 &           1.0000 &           -0.0148 &           0.9998 \\
     &   & 5 &               0.0003 &           1.0000 &           -0.0283 &           1.0000 \\
     &   & 50 &               0.0028 &           1.0000 &            0.0044 &           1.0000 \\
\cline{2-7}
     & \multirow{4}{*}{100} & 2 &              -0.0062 &           0.9879 &           -0.1484 &           0.0152 \\
     &   & 20 &              -0.0229 &           0.7664 &           -0.0449 &           0.8609 \\
     &   & 5 &              -0.0149 &           0.8768 &           -0.0584 &           0.9758 \\
     &   & 50 &              -0.0125 &           0.8440 &           -0.0256 &           0.9879 \\
\cline{2-7}
     & \multirow{3}{*}{2} & 20 &              -0.0167 &           0.9929 &            0.1035 &           0.3834 \\
     &   & 5 &              -0.0087 &           0.9991 &            0.0900 &           0.1772 \\
     &   & 50 &              -0.0063 &           0.9981 &            0.1227 &           0.1379 \\
\cline{2-7}
     & \multirow{2}{*}{20} & 5 &               0.0080 &           1.0000 &           -0.0135 &           0.9997 \\
     &   & 50 &               0.0104 &           1.0000 &            0.0193 &           0.9987 \\
\cline{2-7}
     & 5 & 50 &               0.0024 &           1.0000 &            0.0327 &           1.0000 \\
\cline{1-7}
\multirow{15}{*}{1000} & \multirow{5}{*}{10} & 100 &               0.0307 &           0.6025 &           -0.0039 &           1.0000 \\
     &   & 2 &              -0.0022 &           0.9995 &           -0.0688 &           0.5776 \\
     &   & 20 &               0.0036 &           1.0000 &           -0.0359 &           0.9845 \\
     &   & 5 &              -0.0074 &           0.9051 &           -0.0555 &           0.4539 \\
     &   & 50 &               0.0080 &           1.0000 &           -0.0355 &           0.6025 \\
\cline{2-7}
     & \multirow{4}{*}{100} & 2 &              -0.0329 &           0.3180 &           -0.0649 &           0.4299 \\
     &   & 20 &              -0.0271 &           0.5776 &           -0.0319 &           0.9485 \\
     &   & 5 &              -0.0381 &           0.0588 &           -0.0516 &           0.3180 \\
     &   & 50 &              -0.0227 &           0.6757 &           -0.0316 &           0.4539 \\
\cline{2-7}
     & \multirow{3}{*}{2} & 20 &               0.0058 &           0.9997 &            0.0330 &           0.9640 \\
     &   & 5 &              -0.0052 &           0.9906 &            0.0133 &           1.0000 \\
     &   & 50 &               0.0102 &           0.9981 &            0.0333 &           1.0000 \\
\cline{2-7}
     & \multirow{2}{*}{20} & 5 &              -0.0110 &           0.9176 &           -0.0197 &           0.9176 \\
     &   & 50 &               0.0044 &           1.0000 &            0.0003 &           0.9703 \\
\cline{2-7}
     & 5 & 50 &               0.0153 &           0.8609 &            0.0200 &           1.0000 \\






==> tables/latex/nemenyi_test/dpf_test_path.tex <==
\toprule
     &               &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{RMSE} \\
     &               &       &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Param 1 & Param 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{DPF}{test paths}} \label{tab:nemenyi_dpf_test_path} \\ 
\endlastfoot
\multirow{15}{*}{10} & \multirow{5}{*}{Conditional} & Ones &      \textbf{1.0392} &  \textbf{0.0000} &  \textbf{-0.2413} &  \textbf{0.0000} \\
     &               & Random &      \textbf{0.6055} &  \textbf{0.0000} &  \textbf{-0.1644} &  \textbf{0.0003} \\
     &               & Two stage &      \textbf{1.2704} &  \textbf{0.0000} &  \textbf{-0.2645} &  \textbf{0.0000} \\
     &               & Unconditional &      \textbf{1.1626} &  \textbf{0.0000} &  \textbf{-0.2435} &  \textbf{0.0000} \\
     &               & Zeros &               0.1129 &           0.9879 &           -0.0881 &           0.2239 \\
\cline{2-7}
     & \multirow{4}{*}{Ones} & Random &     \textbf{-0.4337} &  \textbf{0.0005} &            0.0769 &           0.2075 \\
     &               & Two stage &               0.2312 &           0.8261 &           -0.0232 &           1.0000 \\
     &               & Unconditional &               0.1234 &           0.9879 &           -0.0021 &           0.9987 \\
     &               & Zeros &     \textbf{-0.9263} &  \textbf{0.0000} &   \textbf{0.1533} &  \textbf{0.0003} \\
\cline{2-7}
     & \multirow{3}{*}{Random} & Two stage &      \textbf{0.6649} &  \textbf{0.0000} &           -0.1001 &           0.1772 \\
     &               & Unconditional &      \textbf{0.5571} &  \textbf{0.0000} &           -0.0790 &           0.5028 \\
     &               & Zeros &     \textbf{-0.4926} &  \textbf{0.0000} &            0.0764 &           0.4299 \\
\cline{2-7}
     & \multirow{2}{*}{Two stage} & Unconditional &              -0.1078 &           0.9972 &            0.0211 &           0.9972 \\
     &               & Zeros &     \textbf{-1.1575} &  \textbf{0.0000} &   \textbf{0.1765} &  \textbf{0.0002} \\
\cline{2-7}
     & Unconditional & Zeros &     \textbf{-1.0497} &  \textbf{0.0000} &            0.1554 &           0.0023 \\
\cline{1-7}
\multirow{15}{*}{100} & \multirow{5}{*}{Conditional} & Ones &               0.0369 &           0.7872 &  \textbf{-0.1604} &  \textbf{0.0001} \\
     &               & Random &               0.0150 &           0.9906 &           -0.0855 &           0.7224 \\
     &               & Two stage &              -0.0170 &           0.8071 &           -0.0123 &           0.9991 \\
     &               & Unconditional &               0.0134 &           0.9290 &           -0.0791 &           0.3609 \\
     &               & Zeros &              -0.0023 &           1.0000 &           -0.0235 &           0.8915 \\
\cline{2-7}
     & \multirow{4}{*}{Ones} & Random &              -0.0219 &           0.9929 &            0.0749 &           0.0308 \\
     &               & Two stage &              -0.0539 &           0.0720 &   \textbf{0.1481} &  \textbf{0.0006} \\
     &               & Unconditional &              -0.0235 &           0.9999 &            0.0813 &           0.1379 \\
     &               & Zeros &              -0.0391 &           0.8768 &            0.1369 &           0.0104 \\
\cline{2-7}
     & \multirow{3}{*}{Random} & Two stage &              -0.0320 &           0.3391 &            0.0732 &           0.9393 \\
     &               & Unconditional &              -0.0016 &           0.9998 &            0.0064 &           0.9981 \\
     &               & Zeros &              -0.0173 &           0.9981 &            0.0620 &           0.9999 \\
\cline{2-7}
     & \multirow{2}{*}{Two stage} & Unconditional &               0.0304 &           0.1633 &           -0.0668 &           0.6757 \\
     &               & Zeros &               0.0147 &           0.6993 &           -0.0112 &           0.9906 \\
\cline{2-7}
     & Unconditional & Zeros &              -0.0157 &           0.9703 &            0.0556 &           0.9758 \\
\cline{1-7}
\multirow{15}{*}{1000} & \multirow{5}{*}{Conditional} & Ones &              -0.0017 &           1.0000 &           -0.0590 &           0.6993 \\
     &               & Random &               0.0009 &           0.9997 &           -0.0246 &           1.0000 \\
     &               & Two stage &              -0.0103 &           0.8261 &           -0.0273 &           0.9906 \\
     &               & Unconditional &               0.0185 &           0.9929 &           -0.0909 &           0.3609 \\
     &               & Zeros &              -0.0075 &           0.9972 &           -0.0097 &           0.9972 \\
\cline{2-7}
     & \multirow{4}{*}{Ones} & Random &               0.0026 &           1.0000 &            0.0344 &           0.8440 \\
     &               & Two stage &              -0.0086 &           0.9290 &            0.0317 &           0.9805 \\
     &               & Unconditional &               0.0202 &           0.9640 &           -0.0319 &           0.9987 \\
     &               & Zeros &              -0.0059 &           0.9999 &            0.0493 &           0.9567 \\
\cline{2-7}
     & \multirow{3}{*}{Random} & Two stage &              -0.0112 &           0.9640 &           -0.0027 &           0.9991 \\
     &               & Unconditional &               0.0176 &           0.9290 &           -0.0663 &           0.5277 \\
     &               & Zeros &              -0.0084 &           1.0000 &            0.0149 &           0.9999 \\
\cline{2-7}
     & \multirow{2}{*}{Two stage} & Unconditional &               0.0288 &           0.3834 &           -0.0637 &           0.8261 \\
     &               & Zeros &               0.0028 &           0.9879 &            0.0176 &           1.0000 \\
\cline{2-7}
     & Unconditional & Zeros &              -0.0261 &           0.8609 &            0.0812 &           0.7447 \\






==> tables/latex/nemenyi_test/lfrm_finite_20.tex <==
\toprule
      &    &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{Reconstruction error} \\
      &    &       &      Mean difference & P-Value &      Mean difference & P-Value \\
Time & Sampler 1 & Sampler 2 &                      &         &                      &         \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLFRMCaption{K=20}} \label{tab:nemenyi_lfrm_finite_20} \\ 
\endlastfoot
\multirow{3}{*}{100} & \multirow{2}{*}{DPF} & Gibbs &               0.0051 &  0.0011 &               7.2875 &      NS \\
      &    & PG &               0.0024 &  0.9695 &             -57.6125 &      NS \\
\cline{2-7}
      & PG & Gibbs &               0.0026 &  0.0026 &              64.9000 &      NS \\
\cline{1-7}
\multirow{3}{*}{1000} & \multirow{2}{*}{DPF} & Gibbs &               0.0048 &      NS &               8.7000 &      NS \\
      &    & PG &               0.0024 &      NS &              -2.8375 &      NS \\
\cline{2-7}
      & PG & Gibbs &               0.0024 &      NS &              11.5375 &      NS \\
\cline{1-7}
\multirow{3}{*}{10000} & \multirow{2}{*}{DPF} & Gibbs &              -0.0014 &      NS &               0.4000 &      NS \\
      &    & PG &               0.0015 &      NS &              -1.8875 &      NS \\
\cline{2-7}
      & PG & Gibbs &              -0.0029 &      NS &               2.2875 &      NS \\






==> tables/latex/nemenyi_test/lfrm_finite_5.tex <==
\toprule
      &    &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{Reconstruction error} \\
      &    &       &      Mean difference &          P-Value &      Mean difference & P-Value \\
Time & Sampler 1 & Sampler 2 &                      &                  &                      &         \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLFRMCaption{K=5}} \label{tab:nemenyi_lfrm_finite_5} \\ 
\endlastfoot
\multirow{6}{*}{100} & \multirow{3}{*}{DPF} & Gibbs &      \textbf{0.0074} &  \textbf{0.0002} &             -40.6125 &      NS \\
      &    & PG &               0.0038 &           0.3831 &             -16.1375 &      NS \\
      &    & RG &              -0.0006 &           0.9900 &              -2.0500 &      NS \\
\cline{2-7}
      & \multirow{2}{*}{PG} & Gibbs &               0.0036 &           0.0583 &             -24.4750 &      NS \\
      &    & RG &              -0.0045 &           0.2287 &              14.0875 &      NS \\
\cline{2-7}
      & RG & Gibbs &      \textbf{0.0081} &  \textbf{0.0001} &             -38.5625 &      NS \\
\cline{1-7}
\multirow{6}{*}{1000} & \multirow{3}{*}{DPF} & Gibbs &      \textbf{0.0081} &  \textbf{0.0000} &             -31.5625 &      NS \\
      &    & PG &               0.0009 &           0.0681 &              -5.3125 &      NS \\
      &    & RG &              -0.0009 &           0.4940 &               4.0125 &      NS \\
\cline{2-7}
      & \multirow{2}{*}{PG} & Gibbs &               0.0072 &           0.0143 &             -26.2500 &      NS \\
      &    & RG &              -0.0018 &           0.7253 &               9.3250 &      NS \\
\cline{2-7}
      & RG & Gibbs &      \textbf{0.0091} &  \textbf{0.0003} &             -35.5750 &      NS \\
\cline{1-7}
\multirow{6}{*}{10000} & \multirow{3}{*}{DPF} & Gibbs &      \textbf{0.0086} &  \textbf{0.0000} &             -39.3000 &      NS \\
      &    & PG &               0.0010 &           0.3831 &              -9.1125 &      NS \\
      &    & RG &              -0.0006 &           0.9071 &              -9.7125 &      NS \\
\cline{2-7}
      & \multirow{2}{*}{PG} & Gibbs &               0.0076 &           0.0011 &             -30.1875 &      NS \\
      &    & RG &              -0.0016 &           0.7949 &              -0.6000 &      NS \\
\cline{2-7}
      & RG & Gibbs &      \textbf{0.0092} &  \textbf{0.0000} &             -29.5875 &      NS \\






==> tables/latex/nemenyi_test/lfrm_ibp_20.tex <==
\toprule
       &    &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{Reconstruction error} \\
       &    &       &      Mean difference & P-Value &      Mean difference &          P-Value \\
Time & Sampler 1 & Sampler 2 &                      &         &                      &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLFRMCaption{K=20 and an IBP prior}} \label{tab:nemenyi_lfrm_ibp_20} \\ 
\endlastfoot
\multirow{3}{*}{100} & \multirow{2}{*}{DPF} & Gibbs &               0.0028 &      NS &               9.3250 &           0.5345 \\
       &    & PG &               0.0007 &      NS &             -16.4625 &           0.0175 \\
\cline{2-7}
       & PG & Gibbs &               0.0021 &      NS &     \textbf{25.7875} &  \textbf{0.0004} \\
\cline{1-7}
\multirow{3}{*}{1000} & \multirow{2}{*}{DPF} & Gibbs &               0.0013 &      NS &               6.3250 &               NS \\
       &    & PG &              -0.0010 &      NS &              -3.2625 &               NS \\
\cline{2-7}
       & PG & Gibbs &               0.0023 &      NS &               9.5875 &               NS \\
\cline{1-7}
\multirow{3}{*}{100000} & \multirow{2}{*}{DPF} & Gibbs &               0.0002 &      NS &              -4.4125 &               NS \\
       &    & PG &              -0.0004 &      NS &              -6.1000 &               NS \\
\cline{2-7}
       & PG & Gibbs &               0.0006 &      NS &               1.6875 &               NS \\






==> tables/latex/nemenyi_test/lg_finite_20.tex <==
\toprule
      &    &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{RMSE} \\
      &    &       &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Sampler 1 & Sampler 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLGCaption{K=20}} \label{tab:nemenyi_lg_finite_20} \\ 
\endlastfoot
\multirow{3}{*}{100} & \multirow{2}{*}{DPF} & Gibbs &               0.7041 &           0.0307 &           -0.0430 &           0.0246 \\
      &    & PG &      \textbf{8.0163} &  \textbf{0.0000} &  \textbf{-0.1185} &  \textbf{0.0000} \\
\cline{2-7}
      & PG & Gibbs &     \textbf{-7.3122} &  \textbf{0.0000} &   \textbf{0.0754} &  \textbf{0.0004} \\
\cline{1-7}
\multirow{3}{*}{1000} & \multirow{2}{*}{DPF} & Gibbs &      \textbf{4.4600} &  \textbf{0.0000} &  \textbf{-0.1574} &  \textbf{0.0000} \\
      &    & PG &      \textbf{1.8011} &  \textbf{0.0000} &  \textbf{-0.0790} &  \textbf{0.0000} \\
\cline{2-7}
      & PG & Gibbs &      \textbf{2.6589} &  \textbf{0.0000} &           -0.0784 &           0.0015 \\
\cline{1-7}
\multirow{3}{*}{10000} & \multirow{2}{*}{DPF} & Gibbs &      \textbf{5.2375} &  \textbf{0.0000} &  \textbf{-0.1793} &  \textbf{0.0000} \\
      &    & PG &      \textbf{1.8331} &  \textbf{0.0000} &  \textbf{-0.0657} &  \textbf{0.0000} \\
\cline{2-7}
      & PG & Gibbs &      \textbf{3.4044} &  \textbf{0.0000} &  \textbf{-0.1136} &  \textbf{0.0006} \\






==> tables/latex/nemenyi_test/lg_finite_5.tex <==
\toprule
      &    &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{RMSE} \\
      &    &       &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Sampler 1 & Sampler 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLGCaption{K=5}} \label{tab:nemenyi_lg_finite_5} \\ 
\endlastfoot
\multirow{6}{*}{100} & \multirow{3}{*}{DPF} & Gibbs &      \textbf{8.7843} &  \textbf{0.0000} &  \textbf{-0.1836} &  \textbf{0.0000} \\
      &    & PG &      \textbf{7.8931} &  \textbf{0.0000} &  \textbf{-0.1154} &  \textbf{0.0000} \\
      &    & RG &              -0.2859 &           0.9999 &            0.0073 &           0.9948 \\
\cline{2-7}
      & \multirow{2}{*}{PG} & Gibbs &               0.8912 &           0.9736 &           -0.0683 &           0.3831 \\
      &    & RG &     \textbf{-8.1790} &  \textbf{0.0000} &   \textbf{0.1226} &  \textbf{0.0000} \\
\cline{2-7}
      & RG & Gibbs &      \textbf{9.0702} &  \textbf{0.0000} &  \textbf{-0.1909} &  \textbf{0.0000} \\
\cline{1-7}
\multirow{6}{*}{1000} & \multirow{3}{*}{DPF} & Gibbs &      \textbf{8.7537} &  \textbf{0.0000} &  \textbf{-0.1851} &  \textbf{0.0000} \\
      &    & PG &      \textbf{6.0201} &  \textbf{0.0000} &  \textbf{-0.0833} &  \textbf{0.0000} \\
      &    & RG &              -0.4225 &           0.9614 &            0.0055 &           0.6499 \\
\cline{2-7}
      & \multirow{2}{*}{PG} & Gibbs &               2.7337 &           0.1589 &           -0.1018 &           0.0209 \\
      &    & RG &     \textbf{-6.4425} &  \textbf{0.0000} &   \textbf{0.0888} &  \textbf{0.0000} \\
\cline{2-7}
      & RG & Gibbs &      \textbf{9.1762} &  \textbf{0.0000} &  \textbf{-0.1906} &  \textbf{0.0000} \\
\cline{1-7}
\multirow{6}{*}{10000} & \multirow{3}{*}{DPF} & Gibbs &      \textbf{9.0712} &  \textbf{0.0000} &  \textbf{-0.1974} &  \textbf{0.0000} \\
      &    & PG &      \textbf{4.3285} &  \textbf{0.0000} &  \textbf{-0.0861} &  \textbf{0.0000} \\
      &    & RG &              -0.0766 &           0.6499 &           -0.0145 &           0.9071 \\
\cline{2-7}
      & \multirow{2}{*}{PG} & Gibbs &               4.7427 &           0.1802 &           -0.1112 &           0.0209 \\
      &    & RG &     \textbf{-4.4052} &  \textbf{0.0000} &   \textbf{0.0716} &  \textbf{0.0000} \\
\cline{2-7}
      & RG & Gibbs &      \textbf{9.1479} &  \textbf{0.0000} &  \textbf{-0.1829} &  \textbf{0.0000} \\






==> tables/latex/nemenyi_test/lg_ibp_20.tex <==
\toprule
       &    &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{RMSE} \\
       &    &       &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Sampler 1 & Sampler 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanLGCaption{K=20 and an IBP prior}} \label{tab:nemenyi_lg_ibp_20} \\ 
\endlastfoot
\multirow{3}{*}{100} & \multirow{2}{*}{DPF} & Gibbs &               1.7953 &           0.9695 &           -0.0275 &           0.4151 \\
       &    & PG &      \textbf{5.0827} &  \textbf{0.0000} &  \textbf{-0.0856} &  \textbf{0.0000} \\
\cline{2-7}
       & PG & Gibbs &     \textbf{-3.2874} &  \textbf{0.0000} &   \textbf{0.0582} &  \textbf{0.0003} \\
\cline{1-7}
\multirow{3}{*}{1000} & \multirow{2}{*}{DPF} & Gibbs &               1.5649 &           0.1180 &  \textbf{-0.0974} &  \textbf{0.0000} \\
       &    & PG &      \textbf{2.7708} &  \textbf{0.0000} &  \textbf{-0.0646} &  \textbf{0.0000} \\
\cline{2-7}
       & PG & Gibbs &     \textbf{-1.2059} &  \textbf{0.0000} &           -0.0328 &           0.7088 \\
\cline{1-7}
\multirow{3}{*}{100000} & \multirow{2}{*}{DPF} & Gibbs &      \textbf{2.4641} &  \textbf{0.0000} &  \textbf{-0.1124} &  \textbf{0.0000} \\
       &    & PG &               1.3703 &           0.0246 &           -0.0334 &           0.0045 \\
\cline{2-7}
       & PG & Gibbs &      \textbf{1.0938} &  \textbf{0.0000} &  \textbf{-0.0790} &  \textbf{0.0008} \\






==> tables/latex/nemenyi_test/pg_annealing_power.tex <==
\toprule
     &     &     & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{RMSE} \\
     &     &     &      Mean difference &          P-Value &  Mean difference &          P-Value \\
Time & Param 1 & Param 2 &                      &                  &                  &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{PG}{annealing powers}} \label{tab:nemenyi_pg_annealing_power} \\ 
\endlastfoot
\multirow{6}{*}{10} & \multirow{3}{*}{0.0} & 1.0 &     \textbf{-0.8443} &  \textbf{0.0000} &           0.1910 &           0.0051 \\
     &     & 2.0 &     \textbf{-0.9463} &  \textbf{0.0000} &  \textbf{0.2878} &  \textbf{0.0000} \\
     &     & 3.0 &     \textbf{-0.8237} &  \textbf{0.0000} &  \textbf{0.2481} &  \textbf{0.0000} \\
\cline{2-7}
     & \multirow{2}{*}{1.0} & 2.0 &              -0.1019 &           0.0703 &           0.0968 &           0.0264 \\
     &     & 3.0 &               0.0206 &           0.9565 &           0.0571 &           0.1991 \\
\cline{2-7}
     & 2.0 & 3.0 &               0.1226 &           0.3172 &          -0.0397 &           0.9307 \\
\cline{1-7}
\multirow{6}{*}{100} & \multirow{3}{*}{0.0} & 1.0 &     \textbf{-0.2557} &  \textbf{0.0000} &  \textbf{0.1933} &  \textbf{0.0003} \\
     &     & 2.0 &     \textbf{-0.3468} &  \textbf{0.0000} &  \textbf{0.2685} &  \textbf{0.0000} \\
     &     & 3.0 &     \textbf{-0.3332} &  \textbf{0.0000} &  \textbf{0.2875} &  \textbf{0.0000} \\
\cline{2-7}
     & \multirow{2}{*}{1.0} & 2.0 &              -0.0911 &           0.0020 &           0.0752 &           0.5298 \\
     &     & 3.0 &              -0.0775 &           0.0617 &           0.0941 &           0.1448 \\
\cline{2-7}
     & 2.0 & 3.0 &               0.0136 &           0.8319 &           0.0189 &           0.9446 \\
\cline{1-7}
\multirow{6}{*}{1000} & \multirow{3}{*}{0.0} & 1.0 &     \textbf{-0.1944} &  \textbf{0.0000} &           0.1463 &           0.0703 \\
     &     & 2.0 &     \textbf{-0.2415} &  \textbf{0.0000} &  \textbf{0.2825} &  \textbf{0.0000} \\
     &     & 3.0 &     \textbf{-0.2380} &  \textbf{0.0000} &  \textbf{0.3128} &  \textbf{0.0000} \\
\cline{2-7}
     & \multirow{2}{*}{1.0} & 2.0 &              -0.0471 &           0.1615 &           0.1362 &           0.0141 \\
     &     & 3.0 &              -0.0436 &           0.7219 &  \textbf{0.1666} &  \textbf{0.0006} \\
\cline{2-7}
     & 2.0 & 3.0 &               0.0034 &           0.8555 &           0.0303 &           0.9148 \\






==> tables/latex/nemenyi_test/pg_num_particles.tex <==
\toprule
     &   &    & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{RMSE} \\
     &   &    &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Param 1 & Param 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{PG}{number of particles}} \label{tab:nemenyi_pg_num_particles} \\ 
\endlastfoot
\multirow{15}{*}{10} & \multirow{5}{*}{10} & 100 &      \textbf{2.7480} &  \textbf{0.0000} &  \textbf{-0.5587} &  \textbf{0.0000} \\
     &   & 2 &              -0.2048 &           0.5277 &            0.0359 &           0.9929 \\
     &   & 20 &               0.3871 &           0.0245 &           -0.0349 &           0.9845 \\
     &   & 5 &              -0.1429 &           0.6517 &           -0.0092 &           1.0000 \\
     &   & 50 &      \textbf{1.4779} &  \textbf{0.0000} &  \textbf{-0.2271} &  \textbf{0.0001} \\
\cline{2-7}
     & \multirow{4}{*}{100} & 2 &     \textbf{-2.9527} &  \textbf{0.0000} &   \textbf{0.5946} &  \textbf{0.0000} \\
     &   & 20 &     \textbf{-2.3609} &  \textbf{0.0000} &   \textbf{0.5238} &  \textbf{0.0000} \\
     &   & 5 &     \textbf{-2.8909} &  \textbf{0.0000} &   \textbf{0.5495} &  \textbf{0.0000} \\
     &   & 50 &              -1.2701 &           0.0477 &   \textbf{0.3316} &  \textbf{0.0001} \\
\cline{2-7}
     & \multirow{3}{*}{2} & 20 &      \textbf{0.5918} &  \textbf{0.0000} &           -0.0707 &           0.7447 \\
     &   & 5 &               0.0619 &           1.0000 &           -0.0450 &           0.9981 \\
     &   & 50 &      \textbf{1.6826} &  \textbf{0.0000} &  \textbf{-0.2630} &  \textbf{0.0000} \\
\cline{2-7}
     & \multirow{2}{*}{20} & 5 &     \textbf{-0.5300} &  \textbf{0.0000} &            0.0257 &           0.9640 \\
     &   & 50 &      \textbf{1.0908} &  \textbf{0.0000} &           -0.1922 &           0.0031 \\
\cline{2-7}
     & 5 & 50 &      \textbf{1.6208} &  \textbf{0.0000} &  \textbf{-0.2179} &  \textbf{0.0000} \\
\cline{1-7}
\multirow{15}{*}{100} & \multirow{5}{*}{10} & 100 &               0.1149 &           0.0477 &            0.0470 &               NS \\
     &   & 2 &              -0.0446 &           0.3834 &            0.0728 &               NS \\
     &   & 20 &               0.0268 &           0.9879 &            0.0589 &               NS \\
     &   & 5 &              -0.0005 &           1.0000 &            0.0379 &               NS \\
     &   & 50 &               0.0207 &           0.9845 &            0.1246 &               NS \\
\cline{2-7}
     & \multirow{4}{*}{100} & 2 &     \textbf{-0.1595} &  \textbf{0.0000} &            0.0258 &               NS \\
     &   & 20 &              -0.0881 &           0.2976 &            0.0119 &               NS \\
     &   & 5 &              -0.1154 &           0.0218 &           -0.0092 &               NS \\
     &   & 50 &              -0.0942 &           0.3180 &            0.0776 &               NS \\
\cline{2-7}
     & \multirow{3}{*}{2} & 20 &               0.0713 &           0.0720 &           -0.0139 &               NS \\
     &   & 5 &               0.0441 &           0.5526 &           -0.0350 &               NS \\
     &   & 50 &               0.0653 &           0.0651 &            0.0518 &               NS \\
\cline{2-7}
     & \multirow{2}{*}{20} & 5 &              -0.0272 &           0.9485 &           -0.0211 &               NS \\
     &   & 50 &              -0.0061 &           1.0000 &            0.0657 &               NS \\
\cline{2-7}
     & 5 & 50 &               0.0212 &           0.9393 &            0.0867 &               NS \\
\cline{1-7}
\multirow{15}{*}{1000} & \multirow{5}{*}{10} & 100 &               0.0185 &           0.5776 &           -0.0345 &               NS \\
     &   & 2 &              -0.0104 &           1.0000 &           -0.0136 &               NS \\
     &   & 20 &               0.0113 &           0.5776 &           -0.0082 &               NS \\
     &   & 5 &               0.0154 &           0.9998 &            0.0311 &               NS \\
     &   & 50 &               0.0055 &           1.0000 &           -0.0106 &               NS \\
\cline{2-7}
     & \multirow{4}{*}{100} & 2 &              -0.0289 &           0.6025 &            0.0209 &               NS \\
     &   & 20 &              -0.0071 &           1.0000 &            0.0263 &               NS \\
     &   & 5 &              -0.0030 &           0.8071 &            0.0656 &               NS \\
     &   & 50 &              -0.0129 &           0.6517 &            0.0239 &               NS \\
\cline{2-7}
     & \multirow{3}{*}{2} & 20 &               0.0218 &           0.6025 &            0.0054 &               NS \\
     &   & 5 &               0.0259 &           0.9999 &            0.0447 &               NS \\
     &   & 50 &               0.0160 &           1.0000 &            0.0030 &               NS \\
\cline{2-7}
     & \multirow{2}{*}{20} & 5 &               0.0041 &           0.8071 &            0.0393 &               NS \\
     &   & 50 &              -0.0058 &           0.6517 &           -0.0024 &               NS \\
\cline{2-7}
     & 5 & 50 &              -0.0099 &           1.0000 &           -0.0417 &               NS \\






==> tables/latex/nemenyi_test/pg_resample_threshold.tex <==
\toprule
     &      &     & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{RMSE} \\
     &      &     &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Param 1 & Param 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{PG}{resampling thresholds}} \label{tab:nemenyi_pg_resample_threshold} \\ 
\endlastfoot
\multirow{10}{*}{10} & \multirow{4}{*}{0.0} & 0.25 &              -0.0913 &           0.9846 &           -0.0222 &           0.9740 \\
     &      & 0.5 &              -0.0146 &           1.0000 &           -0.0581 &           0.3502 \\
     &      & 0.75 &              -0.0197 &           1.0000 &           -0.0552 &           0.7304 \\
     &      & 1.0 &      \textbf{0.5900} &  \textbf{0.0000} &  \textbf{-0.1732} &  \textbf{0.0000} \\
\cline{2-7}
     & \multirow{3}{*}{0.25} & 0.5 &               0.0767 &           0.9885 &           -0.0359 &           0.8245 \\
     &      & 0.75 &               0.0716 &           0.9671 &           -0.0330 &           0.9885 \\
     &      & 1.0 &      \textbf{0.6813} &  \textbf{0.0000} &  \textbf{-0.1510} &  \textbf{0.0006} \\
\cline{2-7}
     & \multirow{2}{*}{0.5} & 0.75 &              -0.0051 &           1.0000 &            0.0029 &           0.9916 \\
     &      & 1.0 &      \textbf{0.6047} &  \textbf{0.0000} &           -0.1152 &           0.0467 \\
\cline{2-7}
     & 0.75 & 1.0 &      \textbf{0.6097} &  \textbf{0.0000} &           -0.1180 &           0.0070 \\
\cline{1-7}
\multirow{10}{*}{100} & \multirow{4}{*}{0.0} & 0.25 &               0.0173 &           0.7797 &           -0.0516 &               NS \\
     &      & 0.5 &               0.0330 &           0.5100 &           -0.0577 &               NS \\
     &      & 0.75 &               0.0300 &           0.8643 &           -0.0361 &               NS \\
     &      & 1.0 &      \textbf{0.1700} &  \textbf{0.0000} &           -0.1385 &               NS \\
\cline{2-7}
     & \multirow{3}{*}{0.25} & 0.5 &               0.0158 &           0.9983 &           -0.0062 &               NS \\
     &      & 0.75 &               0.0127 &           1.0000 &            0.0155 &               NS \\
     &      & 1.0 &      \textbf{0.1528} &  \textbf{0.0001} &           -0.0869 &               NS \\
\cline{2-7}
     & \multirow{2}{*}{0.5} & 0.75 &              -0.0030 &           0.9916 &            0.0217 &               NS \\
     &      & 1.0 &      \textbf{0.1370} &  \textbf{0.0008} &           -0.0807 &               NS \\
\cline{2-7}
     & 0.75 & 1.0 &      \textbf{0.1400} &  \textbf{0.0001} &           -0.1024 &               NS \\
\cline{1-7}
\multirow{10}{*}{1000} & \multirow{4}{*}{0.0} & 0.25 &               0.0507 &           0.0414 &           -0.0787 &           0.2196 \\
     &      & 0.5 &               0.0312 &           0.4010 &           -0.0618 &           0.7797 \\
     &      & 0.75 &               0.0466 &           0.0664 &           -0.0985 &           0.0527 \\
     &      & 1.0 &      \textbf{0.1380} &  \textbf{0.0000} &           -0.1780 &           0.0017 \\
\cline{2-7}
     & \multirow{3}{*}{0.25} & 0.5 &              -0.0195 &           0.9134 &            0.0168 &           0.9390 \\
     &      & 0.75 &              -0.0041 &           1.0000 &           -0.0198 &           0.9916 \\
     &      & 1.0 &               0.0873 &           0.0020 &           -0.0993 &           0.5947 \\
\cline{2-7}
     & \multirow{2}{*}{0.5} & 0.75 &               0.0154 &           0.9590 &           -0.0366 &           0.6505 \\
     &      & 1.0 &      \textbf{0.1067} &  \textbf{0.0000} &           -0.1161 &           0.1139 \\
\cline{2-7}
     & 0.75 & 1.0 &               0.0913 &           0.0010 &           -0.0795 &           0.9134 \\






==> tables/latex/nemenyi_test/pg_test_path.tex <==
\toprule
     &               &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{RMSE} \\
     &               &       &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Param 1 & Param 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanTuningCaption{PG}{test paths}} \label{tab:nemenyi_pg_test_path} \\ 
\endlastfoot
\multirow{15}{*}{10} & \multirow{5}{*}{Conditional} & Ones &      \textbf{1.9441} &  \textbf{0.0000} &  \textbf{-0.3619} &  \textbf{0.0000} \\
     &               & Random &      \textbf{1.2298} &  \textbf{0.0000} &  \textbf{-0.2472} &  \textbf{0.0000} \\
     &               & Two stage &      \textbf{1.2831} &  \textbf{0.0000} &  \textbf{-0.1914} &  \textbf{0.0000} \\
     &               & Unconditional &      \textbf{1.2887} &  \textbf{0.0000} &  \textbf{-0.2109} &  \textbf{0.0000} \\
     &               & Zeros &               0.2714 &           0.4539 &           -0.0870 &           0.1055 \\
\cline{2-7}
     & \multirow{4}{*}{Ones} & Random &     \textbf{-0.7143} &  \textbf{0.0000} &            0.1147 &           0.1502 \\
     &               & Two stage &     \textbf{-0.6610} &  \textbf{0.0002} &            0.1705 &           0.0047 \\
     &               & Unconditional &     \textbf{-0.6554} &  \textbf{0.0001} &            0.1510 &           0.0062 \\
     &               & Zeros &     \textbf{-1.6727} &  \textbf{0.0000} &   \textbf{0.2749} &  \textbf{0.0000} \\
\cline{2-7}
     & \multirow{3}{*}{Random} & Two stage &               0.0533 &           0.9998 &            0.0558 &           0.9176 \\
     &               & Unconditional &               0.0589 &           1.0000 &            0.0362 &           0.9393 \\
     &               & Zeros &     \textbf{-0.9584} &  \textbf{0.0000} &            0.1602 &           0.0011 \\
\cline{2-7}
     & \multirow{2}{*}{Two stage} & Unconditional &               0.0056 &           1.0000 &           -0.0195 &           1.0000 \\
     &               & Zeros &     \textbf{-1.0117} &  \textbf{0.0000} &            0.1044 &           0.0588 \\
\cline{2-7}
     & Unconditional & Zeros &     \textbf{-1.0173} &  \textbf{0.0000} &            0.1239 &           0.0477 \\
\cline{1-7}
\multirow{15}{*}{100} & \multirow{5}{*}{Conditional} & Ones &      \textbf{0.5421} &  \textbf{0.0000} &  \textbf{-0.1969} &  \textbf{0.0000} \\
     &               & Random &      \textbf{0.2535} &  \textbf{0.0000} &  \textbf{-0.1982} &  \textbf{0.0002} \\
     &               & Two stage &              -0.0286 &           0.3834 &            0.0011 &           1.0000 \\
     &               & Unconditional &               0.1017 &           0.1156 &           -0.1003 &           0.4064 \\
     &               & Zeros &               0.0404 &           0.9393 &           -0.0214 &           0.9845 \\
\cline{2-7}
     & \multirow{4}{*}{Ones} & Random &              -0.2886 &           0.0345 &           -0.0013 &           0.9998 \\
     &               & Two stage &     \textbf{-0.5707} &  \textbf{0.0000} &   \textbf{0.1981} &  \textbf{0.0000} \\
     &               & Unconditional &     \textbf{-0.4403} &  \textbf{0.0000} &            0.0966 &           0.0794 \\
     &               & Zeros &     \textbf{-0.5017} &  \textbf{0.0000} &            0.1755 &           0.0013 \\
\cline{2-7}
     & \multirow{3}{*}{Random} & Two stage &     \textbf{-0.2821} &  \textbf{0.0000} &   \textbf{0.1993} &  \textbf{0.0002} \\
     &               & Unconditional &              -0.1517 &           0.0062 &            0.0979 &           0.1919 \\
     &               & Zeros &     \textbf{-0.2131} &  \textbf{0.0000} &            0.1768 &           0.0054 \\
\cline{2-7}
     & \multirow{2}{*}{Two stage} & Unconditional &      \textbf{0.1303} &  \textbf{0.0001} &           -0.1015 &           0.4064 \\
     &               & Zeros &               0.0690 &           0.0308 &           -0.0226 &           0.9845 \\
\cline{2-7}
     & Unconditional & Zeros &              -0.0614 &           0.6993 &            0.0789 &           0.8915 \\
\cline{1-7}
\multirow{15}{*}{1000} & \multirow{5}{*}{Conditional} & Ones &      \textbf{0.1854} &  \textbf{0.0000} &  \textbf{-0.1978} &  \textbf{0.0006} \\
     &               & Random &      \textbf{0.1033} &  \textbf{0.0000} &  \textbf{-0.2113} &  \textbf{0.0001} \\
     &               & Two stage &              -0.0091 &           0.9981 &           -0.0177 &           1.0000 \\
     &               & Unconditional &               0.0219 &           0.9929 &           -0.1663 &           0.0047 \\
     &               & Zeros &               0.0045 &           1.0000 &           -0.0879 &           0.5028 \\
\cline{2-7}
     & \multirow{4}{*}{Ones} & Random &              -0.0820 &           0.5028 &           -0.0135 &           0.9997 \\
     &               & Two stage &     \textbf{-0.1944} &  \textbf{0.0000} &   \textbf{0.1801} &  \textbf{0.0004} \\
     &               & Unconditional &     \textbf{-0.1634} &  \textbf{0.0000} &            0.0315 &           0.9987 \\
     &               & Zeros &     \textbf{-0.1808} &  \textbf{0.0000} &            0.1099 &           0.2411 \\
\cline{2-7}
     & \multirow{3}{*}{Random} & Two stage &     \textbf{-0.1124} &  \textbf{0.0000} &   \textbf{0.1936} &  \textbf{0.0001} \\
     &               & Unconditional &     \textbf{-0.0814} &  \textbf{0.0004} &            0.0450 &           0.9703 \\
     &               & Zeros &     \textbf{-0.0988} &  \textbf{0.0000} &            0.1234 &           0.0961 \\
\cline{2-7}
     & \multirow{2}{*}{Two stage} & Unconditional &               0.0310 &           0.8768 &           -0.1486 &           0.0036 \\
     &               & Zeros &               0.0136 &           0.9987 &           -0.0702 &           0.4539 \\
\cline{2-7}
     & Unconditional & Zeros &              -0.0174 &           0.9906 &            0.0784 &           0.5526 \\






==> tables/latex/nemenyi_test/pyclone_finite_12.tex <==
\toprule
      &    &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{B-Cubed F-Measure} \\
      &    &       &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Sampler 1 & Sampler 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanPyCloneCaption{D=10 and K=12}} \label{tab:nemenyi_pyclone_finite_12} \\ 
\endlastfoot
\multirow{3}{*}{100} & \multirow{2}{*}{DPF} & Gibbs &      \textbf{0.2250} &  \textbf{0.0002} &   \textbf{0.1678} &  \textbf{0.0000} \\
      &    & PG &     \textbf{29.3156} &  \textbf{0.0000} &   \textbf{0.4260} &  \textbf{0.0000} \\
\cline{2-7}
      & PG & Gibbs &    \textbf{-29.0906} &  \textbf{0.0000} &           -0.2582 &           0.8022 \\
\cline{1-7}
\multirow{3}{*}{1000} & \multirow{2}{*}{DPF} & Gibbs &               0.3318 &           0.0015 &   \textbf{0.3967} &  \textbf{0.0000} \\
      &    & PG &     \textbf{24.7551} &  \textbf{0.0000} &   \textbf{0.6541} &  \textbf{0.0000} \\
\cline{2-7}
      & PG & Gibbs &    \textbf{-24.4233} &  \textbf{0.0000} &  \textbf{-0.2574} &  \textbf{0.0002} \\
\cline{1-7}
\multirow{3}{*}{10000} & \multirow{2}{*}{DPF} & Gibbs &      \textbf{0.3240} &  \textbf{0.0000} &   \textbf{0.4466} &  \textbf{0.0000} \\
      &    & PG &     \textbf{13.4891} &  \textbf{0.0000} &   \textbf{0.5367} &  \textbf{0.0000} \\
\cline{2-7}
      & PG & Gibbs &    \textbf{-13.1651} &  \textbf{0.0000} &           -0.0902 &           0.0379 \\






==> tables/latex/nemenyi_test/pyclone_finite_4.tex <==
\toprule
      &    &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{B-Cubed F-Measure} \\
      &    &       &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Sampler 1 & Sampler 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanPyCloneCaption{D=4 and K=4}} \label{tab:nemenyi_pyclone_finite_4} \\ 
\endlastfoot
\multirow{6}{*}{100} & \multirow{3}{*}{DPF} & Gibbs &      \textbf{0.9702} &  \textbf{0.0000} &   \textbf{0.2967} &  \textbf{0.0000} \\
      &    & PG &     \textbf{92.2997} &  \textbf{0.0000} &   \textbf{0.6791} &  \textbf{0.0000} \\
      &    & RG &              -0.0144 &           0.2559 &           -0.0303 &           0.4940 \\
\cline{2-7}
      & \multirow{2}{*}{PG} & Gibbs &    \textbf{-91.3295} &  \textbf{0.0000} &  \textbf{-0.3824} &  \textbf{0.0000} \\
      &    & RG &    \textbf{-92.3141} &  \textbf{0.0000} &  \textbf{-0.7093} &  \textbf{0.0000} \\
\cline{2-7}
      & RG & Gibbs &      \textbf{0.9845} &  \textbf{0.0000} &   \textbf{0.3270} &  \textbf{0.0000} \\
\cline{1-7}
\multirow{6}{*}{1000} & \multirow{3}{*}{DPF} & Gibbs &      \textbf{0.9738} &  \textbf{0.0000} &   \textbf{0.3128} &  \textbf{0.0000} \\
      &    & PG &     \textbf{89.3427} &  \textbf{0.0000} &   \textbf{0.6741} &  \textbf{0.0000} \\
      &    & RG &              -0.0116 &           1.0000 &           -0.0270 &           0.9282 \\
\cline{2-7}
      & \multirow{2}{*}{PG} & Gibbs &    \textbf{-88.3689} &  \textbf{0.0000} &  \textbf{-0.3614} &  \textbf{0.0000} \\
      &    & RG &    \textbf{-89.3544} &  \textbf{0.0000} &  \textbf{-0.7012} &  \textbf{0.0000} \\
\cline{2-7}
      & RG & Gibbs &      \textbf{0.9854} &  \textbf{0.0000} &   \textbf{0.3398} &  \textbf{0.0000} \\
\cline{1-7}
\multirow{6}{*}{10000} & \multirow{3}{*}{DPF} & Gibbs &      \textbf{0.9813} &  \textbf{0.0000} &   \textbf{0.3402} &  \textbf{0.0000} \\
      &    & PG &     \textbf{85.0018} &  \textbf{0.0000} &   \textbf{0.6797} &  \textbf{0.0000} \\
      &    & RG &              -0.0084 &           0.9948 &           -0.0083 &           0.9900 \\
\cline{2-7}
      & \multirow{2}{*}{PG} & Gibbs &    \textbf{-84.0205} &  \textbf{0.0001} &  \textbf{-0.3395} &  \textbf{0.0000} \\
      &    & RG &    \textbf{-85.0103} &  \textbf{0.0000} &  \textbf{-0.6879} &  \textbf{0.0000} \\
\cline{2-7}
      & RG & Gibbs &      \textbf{0.9898} &  \textbf{0.0000} &   \textbf{0.3484} &  \textbf{0.0000} \\






==> tables/latex/nemenyi_test/pyclone_finite_8.tex <==
\toprule
      &    &       & \multicolumn{2}{c}{Relative log density} & \multicolumn{2}{c}{B-Cubed F-Measure} \\
      &    &       &      Mean difference &          P-Value &   Mean difference &          P-Value \\
Time & Sampler 1 & Sampler 2 &                      &                  &                   &                  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\\ 
\caption{\friedmanPyCloneCaption{D=10 and K=8}} \label{tab:nemenyi_pyclone_finite_8} \\ 
\endlastfoot
\multirow{3}{*}{100} & \multirow{2}{*}{DPF} & Gibbs &      \textbf{0.4032} &  \textbf{0.0000} &   \textbf{0.4152} &  \textbf{0.0000} \\
      &    & PG &     \textbf{60.3425} &  \textbf{0.0000} &   \textbf{0.7977} &  \textbf{0.0000} \\
\cline{2-7}
      & PG & Gibbs &    \textbf{-59.9393} &  \textbf{0.0000} &           -0.3825 &           0.2207 \\
\cline{1-7}
\multirow{3}{*}{1000} & \multirow{2}{*}{DPF} & Gibbs &      \textbf{0.4452} &  \textbf{0.0000} &   \textbf{0.5236} &  \textbf{0.0000} \\
      &    & PG &     \textbf{58.3945} &  \textbf{0.0000} &   \textbf{0.9094} &  \textbf{0.0000} \\
\cline{2-7}
      & PG & Gibbs &    \textbf{-57.9493} &  \textbf{0.0000} &           -0.3858 &           0.0568 \\
\cline{1-7}
\multirow{3}{*}{10000} & \multirow{2}{*}{DPF} & Gibbs &      \textbf{0.4391} &  \textbf{0.0000} &   \textbf{0.5242} &  \textbf{0.0000} \\
      &    & PG &     \textbf{53.8505} &  \textbf{0.0000} &   \textbf{0.8962} &  \textbf{0.0000} \\
\cline{2-7}
      & PG & Gibbs &    \textbf{-53.4114} &  \textbf{0.0000} &  \textbf{-0.3719} &  \textbf{0.0000} \\





